Spatial structure of shock formation

The formation of a singularity in a compressible gas, as described by the Euler equation, is characterized by the steepening, and eventual overturning of a wave. Using a self-similar description in two space dimensions, we show that the spatial structure of this process, which starts at a point, is equivalent to the formation of a caustic, i.e. to a cusp catastrophe. The lines along which the profile has infinite slope correspond to the caustic lines, from which we construct the position of the shock. By solving the similarity equation, we obtain a complete local description of wave steepening and of the spreading of the shock from a point.

==> plane_fig <==
#FIG 3.2  Produced by xfig version 3.2.5b
Landscape
Center
Inches
Letter  
100.00
Single
-2
1200 2
2 1 0 1 0 7 48 -1 -1 0.000 0 0 -1 0 0 2
	 7800 6825 8475 6825
2 5 0 1 0 -1 49 -1 -1 0.000 0 0 -1 0 0 5
	0 plane_cleaned.jpg
	 3225 2250 13395 2250 13395 8250 3225 8250 3225 2250
4 0 0 48 -1 0 15 0.0000 4 165 705 6300 4725 size of \001
4 0 0 48 -1 0 15 0.0000 4 165 540 6300 4980 cloud\001
4 0 0 48 -1 0 15 0.0000 4 165 585 9450 8325 time t\001
4 0 0 48 -1 0 15 0.0000 4 165 615 8625 6900 fit A t\001
4 0 0 48 -1 0 10 0.0000 4 105 195 9225 6750 1/2\001

